Capacitated spatial clustering with multiple constraints and attributes

Capacitated spatial clustering, a type of unsupervised machine learning method, is often used to tackle problems in compressing, classifying, logistic optimization and infrastructure optimization. Depending on the application at hand, a wide set of extensions may be necessary in clustering. In this article we propose a number of novel extensions to PACK that is a novel capacitated spatial clustering method. These extensions are relocation and location preference of cluster centers, outliers, and non-spatial attributes. The strength of PACK is that it can consider all of these extensions jointly. We demonstrate the usefulness PACK with a real world example in edge computing server placement for a city region with various different set ups, where we take into consideration outliers, center placement, and non-spatial attributes. Different setups are evaluated with summary statistics on spatial proximity and attribute similarity. As a result, the similarity of the clusters was improved at best by 53%, while simultaneously the proximity degraded only 18%. In alternate scenarios, both proximity and similarity were improved. The different extensions proved to provide a valuable way to include non-spatial information into the cluster analysis, and attain better overall proximity and similarity. Furthermore, we provide easy-to-use software tools (rpack) for conducting clustering analyses.

==> text/AppA_Cap_clustering.tex <==

\section*{Appendix A: Capacitated clustering}
\label{app_frameworks}

We start by formulating partitional clustering as an optimization problem, and then continue by considering the connection to model-based clustering.

\subsection*{Partitional clustering}
Given a data set of $n$ points, let  $x_i=[x_{i1}, x_{i2}]$ be the spatial coordinates of  a point $i$.  %The weight may represent for example the number of duplicate points or the amount of demand (See further information in Section~\ref{weights}).
We denote by $c_j=[c_{j1}, c_{j2}]$, $j=1,\dots,k$ the coordinates for the $k$ cluster centers (heads). %For unifying the terminology, we will refer to $c_j$ as centers. 
The distance between a point $i$ and a center $j$ is denoted by   $d(x_i, c_j)$. In addition, let us further denote by $y_{i j}$ the membership of a point $i$ to the center $j$, where $y_{ij}$ equals one if the point $i$ belongs to the cluster $j$ and zero otherwise. 

%In both frameworks, %
The aim is to minimize the sum of the distances between points and the centers they are assigned to. Thus, we consider the  objective function
%Our aim is to locate cluster heads and allocate points to clusters by minimizing a loss function
\begin{equation}
\label{loss}
\argmin_{c_j, y_{i j}} \sum_{i = 1}^{n} \sum_{j = 1}^{k} d(x_i, c_j) y_{i j},% +\lambda  \sum_{i = 1}^{n}  y_{i, k+1}
\end{equation}
with the following two constraints: 
\begin{equation}
 \label{const2}
    % Membership
    y_{i j} \in \{0, 1\} \quad \forall i,j,
\end{equation}
\begin{equation}  
 \label{const3}
\sum_{j = 1}^{k} y_{i j} = 1 \quad \forall i.  \\
\end{equation}
 The constraint (\ref{const2}) dictates that a point $i$ is either assigned to cluster $j$ or not and constraint (\ref{const3}) ensures that each point is assigned to exactly one cluster.


\subsection*{Model-based clustering }
\label{frameworks_intersection}

We consider two approaches to model-based clustering, the mixture model approach and the classification maximum likelihood approach. 

\subsubsection*{Mixture-models}
In a mixture model \citep[see e.g.][]{McLachlan00}, data is assumed to have emerged from a mixture of parametric density family
\begin{equation}
\label{mixture}
f(x)=\sum_{j=1}^kf(x|\theta_j)p(\pi_j),
\end{equation}
where $f(x|\theta_j)$ is the density function of a data point $x$ given that it has emerged from cluster $j$ and $p(\pi_j)$ is the probability of observing a data point from cluster $j$. The number of clusters $k$ is predetermined.  This corresponds to a data generating process where
\[
\begin{split}
z_i&\sim \text{Multinom}(1,[\pi_1,\dots,\pi_k]) \\
x_i|z_i &\sim f(\cdot|\theta_{z_i}),
\end{split}
\]
for each $x_i$, $i=1,\dots,n$.


Given a data set $x_1,\dots,x_n$, the aim is to estimate the parameter vectors $\theta=[\theta_1,\dots,\theta_k]$ and $\pi=[\pi_1,\dots,\pi_k]$ by maximizing the logarithm of the likelihood function
\begin{equation}
\label{mixture_ml}
l(\theta,\pi;x_1,\dots,x_n) =  \sum_{i=1}^n \log \sum_{j=1}^k \pi_j f(x_i|\theta_j). 
\end{equation}
 Each point $x_i$ is then assigned with a probability  of belonging to each cluster $j$. The data set $x_1,\dots,x_n$ can then be clustered by assigning each $x_i$ to the cluster with the highest likelihood. See \cite{Fraley02} for further information.    

%A well known special case are the Gaussian mixture models (GMM) obtained using the Gaussian distributions.

Maximizing the log-likelihood of the mixture model (\ref{mixture_ml}) can be connected to the minimization problem (\ref{loss}) when specific assumptions are made regarding the distance $d$, the parameters $\theta_j$ and proportions $\pi_j$ of the mixture densities. For example, if the distance $d$ is measured with a squared Euclidean distance metric, it can be shown that the minimization of (\ref{loss}) corresponds to estimating the parameters of an isotropic (i.e., spherical) Gaussian mixture model where each cluster is assumed to have the same proportion $\pi_j$  and the cluster variances tend to zero \citep[see e.g.][] {Bishop06}. This result is known as the small variance asymptotic derivation of K-means clustering \citep{Jiang12}.  


\subsubsection*{Classification maximum likelihood approach}
\label{classification_section}
Let us denote by $P=[P_1,\dots,P_k]$ the partition of the $n$ points into $k$ groups where $P_j$ contains the points assigned to group $j$. These groups correspond to the points assigned to a given facility in location-allocation and points assigned to one cluster in partitional clustering.

In the classification maximum likelihood approach \citep{Celeux92},  this unknown partition $P$ is a parameter vector and the log-likelihood function to be maximized is
\begin{equation}
\label{CML}
l(P,\theta;x_1,\dots,x_n)= \sum_{j=1}^k\sum_{x_i\in P_j} \log f(x_i|\theta_j).
\end{equation}

\citet{Celeux92} use also a more flexible version obtained by incorporating the proportions of clusters $\pi_j$ as follows
\[
\begin{split}
l(P,\theta,\pi;x_1,\dots,x_n)
    &= \sum_{j = 1}^k \sum_{x_i \in P_j} \log \left( \pi_j f(x_i|\theta_j) \right) \\
    &= l(P, \theta;x_1, \dots, x_n) + n_j \log \pi_j,
\end{split}
\]
where $n_j$ is the number of points in the group $j$.
This corresponds to  (\ref{CML}) if the proportions $\pi_j$ are assumed to be equal for each $j=1,\dots,n$. Thus (\ref{CML}) implicitly assumes that the true clusters have equal sizes.

We continue to follow \citet{Celeux92} and explore  the connection between classification maximum likelihood and partitional clustering and location-allocation. Let us assume that $f(\cdot|\theta_j) \sim N(\mu_j, \sigma^2 I)$ for all $j$. Then the classification likelihood is
\begin{equation}
\label{class_ml_Gauss}
\begin{split}
l(P,\mu, \sigma ;x_1, \dots, x_n)
    &= \sum_{j = 1}^k \sum_{x_i \in P_j} \log f(x_i | \theta_j)  \\
    &= \sum_{j = 1}^k \sum_{x_i \in P_j} \left( -\frac{a}{2}\log \sigma^2 -\frac{||x_i - \mu_j||^2}{2 \sigma^2} \right) + c 
\end{split}
\end{equation}
where $a$ is the dimension of data (here $a=2$), and $c$ is a constant independent of $P,\mu$ and $\sigma^2$.

%Following \citet{Celeux92}, we show that maximizing (\ref{class_ml_Gauss}) corresponds to  minimizing 
%\[
%\text{RSS}=\sum_{j=1}^k\sum_{x_i\in C_j} ||x_i-\mu_j||^2 
%\]
%with respect to $C$ and $\mu$.


%https://www.ukessays.com/essays/computer-science/solve-location-allocation-problems-using-genetic-algorithm-computer-science-essay.php

%https://webapps.itc.utwente.nl/librarywww/papers_2011/msc/gfm/arifin.pdf
%Gradu, jossa osa faciliteista fiksattu ja osa voidaan vapauttaa

% https://www.esri.com/about/newsroom/wp-content/uploads/2018/10/solving-a-public-health-problem.pdf
% eli onnistuu requiredina arcgississa


If $\sigma^2$ is known,
\[
    l(\mu,P |\sigma^2, x_1, \dots, x_n) 
        = - \sum_{j = 1}^k \sum_{x_i \in C_j} \left( \frac{||x_i - \mu_j||^2}{2 \sigma^2} \right) + c .
\]
With unknown $\sigma^2$,   it is straightforward to show that (\ref{class_ml_Gauss}) is maximized if  $\sigma^2 = \frac{\text{RSS}}{na}$, where
\begin{equation}
\label{RSS2}
\text{RSS} = \sum_{j = 1}^k \sum_{x_i \in P_j} ||x_i - \mu_j||^2 
\end{equation}
and by plugging it into (\ref{class_ml_Gauss})
\[
    l(\mu,P | x_1, \dots, x_n)  \propto  
        - \log \left( \sum_{j = 1}^k \sum_{x_i \in P_j}||x_i - \mu_j||^2 \right) + c.
\]
Hence, both with known and unknown $\sigma^2$ the classification maximum likelihood with Gaussian distribution corresponds to minimizing (\ref{loss}) with the squared Euclidean distance metric.


On the other hand, if for each cluster, $x_{i1}$ and $x_{i2}$ are independently generated from univariate Laplace  distribution, i.e. $f(\cdot|\theta_j) \sim \text{Laplace}(\mu_j, \sigma I)$ for all $j$,  the classification likelihood function is
\begin{align}
\label{class_ml_Laplace}
%\begin{split}
    l&(P, \mu, \sigma |x_1, \dots, x_n) \nonumber
     = \sum_{j = 1}^k \sum_{x_i \in P_j} \log f(x_i|\theta_j) \nonumber \\
     & = \sum_{j = 1}^k \sum_{x_i \in P_j} \left( -2\log \sigma -\frac{1}{\sigma} 
            \left( |x_{i1} - \mu_{j1}| - |x_{i2} - \mu_{j2}| \right) \right) + c.
%\end{split}
\end{align}

With an analogous reasoning as with the squared Euclidean distance metric, maximizing (\ref{class_ml_Laplace}) is equivalent to minimizing the sum of Manhattan distances
\[
\sum_{j = 1}^k \sum_{x_i \in P_j} |x_{i1} - \mu_{j1}| + |x_{i2} - \mu_{j2}|.
\]
Classification maximum likelihood thus corresponds to solving the clustering problem (\ref{loss}) with the Manhattan distance metric.

Similarly, minimizing (\ref{loss}) with the Euclidean distance metric corresponds to maximizing the  classification maximum likelihood, assuming that the data of each cluster is generated from an isotropic multivariate Laplace distribution defined as a special case of the multivariate exponential power distribution \citep{Naik06,Arslan10} as follows:
\[
    f_j(x) = 
        f (\cdot; \mu_j, \sigma) \propto \frac{1}{\sigma^{a/2}} e^{-\frac{1}{\sigma} \sqrt{(x - \mu_j)^T (x - \mu_j)}}.
\]



==> text/AppB_Tutorial.tex <==
\section*{Appendix B: Tutorial with simulated data}
\label{sim_exp}

This example shows how the capacity constraints guarantee that the workload of different clusters is reasonable. Further, the example illustrates how outliers are identified. We also evaluate clustering extensions with a known cluster structure, using the adjusted Rand index (ARI) \citep{Rand1971} measure.
  
We simulate $500$ data points which form $10$ clusters as follows:

\begin{enumerate}
    \item The number of data points in the simulated clusters is set as $20$, $20$, $40$, $40$, $50$, $50$, $60$, $60$, $80$ and $80$. The uneven cluster sizes illustrate how the results change with and without the capacity limits.

    \item Data points are simulated from a set of multivariate gamma distributions constructed using a normal (Gaussian) copula utilizing the R package \texttt{lcmix} \citep{Song2000}. The shape parameters of the gamma distributions vary between $0$ and $15$, and the scale parameters vary between $0$ and $100$. These parameter values will generate both asymmetric and symmetric clusters.
    
    \item The weights of each data point are generated independently from the uniform distribution $\text{Unif}[1, 100]$. To make clusters less homogeneous in the terms of the weights, about half of the clusters have small weights at the cluster center and heavy weight points at the edge of clusters. These weights are directly proportional to the Euclidean distance  between the cluster center (the mean point of the multivariate gamma distribution) and the data point.
    
    \item Clusters that consist of independently generated data points, drawn from a set of multivariate gamma distributions, frequently overlap. Separating clusters from each other is thus difficult because cluster shapes are unclear. To reduce the overlap of the resulting clusters, the mean of each multivariate gamma distribution is shifted randomly on a predefined grid. Moreover, we use an additional scaling parameter to draw data points closer to the corresponding cluster center to further reduce the overlap of data points. See Fig. \ref{Fig:sim_gam_mixture} for a schematic illustration of this step.
    
    \item Additional outlier points are sampled uniformly from the grid determined by the outermost data points. Like the weights of the ``true'' data points, the weights of the outlier points are sampled independently from the uniform distribution $\text{Unif}[1, 100]$. Overall, $20$ outlier points are added to the data.
    
\end{enumerate}
%
The simulation algorithm we use to generate data points from multivariate Gamma distribution(s) is included in the rpack R-package \citep{rpack}.

\begin{figure}
\centering
\includegraphics[width=0.8\textwidth]{images/simulate_gamma_mixture.png}
\caption{An illustration of the data overlap reduction scheme with three clusters. The mass center of the distributions (black crosses) are selected randomly on the grid. \label{Fig:sim_gam_mixture}}
\end{figure}

We set the number of centers $k$ as $10$. The capacity limits of each cluster are set as $[1587,3587 ]$, that is, $[\Bar{w} - 1000, \Bar{w} + 1000]$, where $\Bar{w} = \sum_i^n w_i/k = 2587$ is the empirical mean of the cluster weights. We set the outlier penalty parameter $\lambda$ as $0.05$ with the squared Euclidean distance metric and as $0.2$ with the Euclidean distance metric to demonstrate how identifying outliers change the resulting clusters. For each data replicate we run the Algorithm~\ref{alt_alg} with $50$ initial values, selected with the k-means++ algorithm. Clustering results are illustrated in Figs. \ref{SimulationFigure1} and \ref{SimulationFigure2}.

Further, we illustrate how capacity constraints and the outlier penalty change the clustering of  data points determined by latent factors, that is, different multivariate gamma distributions and their parametrizations. We run several data simulations and each time examine how the estimated clusters compare with the densities of the underlying multivariate gamma distributions providing the simulated data points. We call these densities the ground truth clusters. We use the adjusted Rand index (ARI), computed with the R package fpc \citep{Vinh.etal2010}, as a diagnostic metric in this simulation example. The closer the ARI is to one, the closer the clusters are to the ground truth clusters. In this example, capacity limits are determined by the empirical mean of the cluster weights, and we use the same outlier penalty parameter values as described above. Averaged ARI measures are determined based on 50 simulation replications. The averaged ARI results are presented in Fig. \ref{RandIndexFigure}. Finally, we note that the averaged ARI values cannot be exactly one due to the overlap of the ground truth clusters.

\subsubsection{Artificial data points clustering results}

Fig. \ref{SimulationFigure1} \textbf{B} clearly demonstrates that without capacity limits the resulting cluster sizes are drastically uneven: the smallest cluster size is $259$, whereas the largest is $5211$. Further, there is a very large cluster with a concentration of data points. %, and the weight of this cluster would be reasonable to divide with the adjacent clusters. %\todo{Tämä lause on nyt irrallinen, mihin viittaa? Korjaa.}
%Moreover, data points in the top-right corner  are classified into a separate small cluster although we apply the bi-criterion approach to identify outliers.(Fig. \ref{SimulationFigure1} \textbf{B})
Using capacity limits, the concentration of data points is divided into more even-sized clusters (Fig. \ref{SimulationFigure1} \textbf{A}). 

\begin{figure}
\centering
\includegraphics[width=\textwidth]{images/Artificial_squared_Euc.png}
\caption{Continuous clustering of $500$ data points with $10$ clusters and the squared Euclidean  distance metric, with capacity limits \textbf{(A)} and without capacity limits \textbf{(B)}. The black crosses denote estimated cluster centers. For \textbf{(A)}, the cluster sizes vary only within the set limits [1587,3587].\label{SimulationFigure1}}
\end{figure}

Further, Fig. \ref{SimulationFigure2} demonstrates how excluding the oultier penalty parameter results in very broad clusters. For example, the identified cluster found in the right upper corner in Fig. \ref{SimulationFigure2} \textbf{A} is very wide and it would be reasonable to consider the outermost data points as outliers. When the penalty is utilized, these outermost points are consistently determined as outliers.

\begin{figure}
\centering
\includegraphics[width=\textwidth]{images/Artificial_Euc.png}
\caption{Continuous clustering of $500$ data points with $10$ clusters and the standard Euclidean  distance metric, with the outlier penalty \textbf{(A)} and without the outlier penalty \textbf{(B)}. The black crosses denote estimated cluster centers. A total of 379 weight points, located on the upper edge of the map, are assigned to the outgroup in \textbf{(A)}. 
\label{SimulationFigure2}}
\end{figure}

The squared Euclidean distance metric, combined with the outlier penalty, seems to produce the largest averaged adjusted Rand indexes (ARI) (Fig. \ref{RandIndexFigure}). ARI represents how data points classified into different clusters coincide with the known clusters of the artificial data points \citep{Hubert1985}. There is no striking difference between the averaged ARI measures while capacity limits are used in the clustering algorithm and when the same data is clustered without the capacity limits. Overall, the inclusion of the outlier penalty and the capacity limits did not produce clusters which would be drastically in contradiction to the mechanism by which the data points are generated. This is a good property because data points are not forced into clusters which would not reflect the true data while capacity constraints are applied.

The difference between the squared Euclidean and the Euclidean distance metrics is very subtle in the continuous setting. Although the resulting clusters are almost identical, it seems the squared Euclidean metric favors more spherical cluster structures. With the Euclidean metric, large clusters of the original data are divided into smaller, less spherical like clusters.

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{images/ARI.png}
    \caption{Adjusted Rand indexes (ARI) based on 50 simulation replications. Clusters determined using squared Euclidean distance ($L_2^2$) in the loss function are illustrated with filled boxplot and clusters determined using Euclidean distance ($L_2$) in the loss function are illustrated with empty boxplots. Notations ``$+$ LU'' and ``$+ \lambda_{\text{out}}$'' denote, respectively, if capacity limits (Lower and Upper) or the outlier penalty were applied in PACK. The squared Euclidean distance metric, combined with the outlier penalty, seems to produce the largest averaged ARI values.}
    \label{RandIndexFigure}
\end{figure}


%%%%%%%%%%%% VANHA %%%%%%%%%%%%
%Simulate data from Laplace and Gaussian mixtures.  Use k-means and k-median for clustering (continuous setting).  Indicate the wrong and right labeled points. 

%Was the performance better if the data and method were comparable?

%Include outliers.  Is k-median more robust as one might expect
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> text/AppC_Slovakia.tex <==
\section*{Appendix D: Recycling center placement}
\label{slov_exp}

The third experiment places a fixed number of recycling centers in the Slovakian city of Partizánske  such that the average road distance between residents and the centers is minimized. The data set \citep{Cebecauer18} includes a distance matrix, listing the road distances between the demand points, and the locations of those demand points. Further, each demand point has a residential population associated with it, which corresponds here to the weight of the point. 

The experiment applies two PACK extensions. First, as only the resulting recycling center locations are in focus, and not the allocations of the residents, we apply fractional membership to speed up the optimization. Second, since placing a recycling center anywhere is not possible, we restrict the possible placement to 50 predefined locations in the city. These locations as well as the demand points can be seen in the left panel of Fig. \ref{slovakia_points}.

To study the effect of the fractional membership on the speed of the algorithm, we analyze the impact of two different capacity limits on the placement in both fractional and hard membership scenarios. We set the wide capacity limits to $[2963, 4962]$ and the tight capacity limits to $[3962, 3963]$. 

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/plot_slovakia_predet_centers.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/plot_slovakia_k12_predet.png}
    \end{subfigure}
    \caption{
    The optimal placement of 12 recycling centers in the region of Partizánske. Left: the data points and  the center location candidates shown as red crosses. Right: The partitioning with fractional membership and capacity limits for each center set to [2963, 4962]. }
    \label{slovakia_points}
\end{figure}

\begin{table}[ht]
\centering
\begin{tabular}{llllll}
  \toprule
Membership & Limits & Mean & 50\% & 95\% & Time (min) \\ 
  \midrule
fractional & wide & 1.15 & 0.86 & 3.25 & 2.15\\ 
  hard & wide & 1.17 & 0.85 & 3.34 & 7.04 \\ 
  fractional & tight & 1.26 & 0.86 & 3.84 & 2.78 \\ 
  hard & tight & 1.26 & 0.86 & 3.84 & 20.54 \\ 
   \midrule
   \label{fixed_scenarios}
\end{tabular}
\caption{Comparison of the mean, median and 95\% quantile distances for the four setups, each with different membership types and capacity limits to Experiment 3.}
    \label{slovakia_table}
\end{table}

The right panel of Fig. \ref{slovakia_points} illustrates the resulting clustering, obtained with fractional membership and wide capacity limits. The overall clustering seems to be reasonable and the recycling center locations are spread out. There is some overlapping of the clusters in the north-west region of the city. This is due to the underlying distance matrix, where some of the points have exactly the same distance to a certain point, even though the distances appear different based on the map. In the city center, the centers are close to each other, which is partly due to the distribution of the population.

The difference between the clusters resulting from fractional and hard membership is minor based on the mean, median an 95\% quantile distances (Table~\ref{slovakia_table}) and based on the clustering results on the map (result not shown). However, the fractional membership scenarios are much faster to run than the hard membership scenarios. With the wide capacity limits, the algorithm was approximately 3 times faster with fractional membership and with tight limits approximately 10 times faster. Furthermore, we tested even tighter limits that allow only one size for clusters. This problem was easily solved with fractional membership, but it was not solvable with the hard membership constraint, as it was not possible to distribute the weights of the demand points evenly to each cluster without dividing individual weights.

% AO on enemmän discukamaa kuin tähän kuuluvaa
%Overall, we explored the location-allocation problem with predefined distance matrix successfully. Two different capacity limits were set with both hard and fractional membership. As the fractional membership can be seen as a relaxation of the hard membership scenario, they were much faster than the hard membership scenarios. Furthermore, in some cases the fractional membership was the only option to ensure that the problem could be solved. 



==> text/AppD_rel_work.tex <==
\section*{Appendix B: Related work on a set of extensions}
\label{app_rel_work}

\textbf{Membership.} Membership refers to the way point are allocated to clusters. The three main membership types are considered in partitional clustering are, hard, overlapping and fractional membership. 

Hard membership refers to the membership used in k-means, where a point is fully assigned to exactly one cluster. Overlapping membership means a point can be fully assigned to several clusters either with hard membership or with uncertain membership \citep[see reviews  by][]{Baadel16, Cir15}. In fractional membership points weight can be divided by multiple clusters. It allows a more flexible allocation of points into clusters than with hard membership in capacitated clustering and In the extreme case, with hard membership, it may even be that the data points can not be partitioned according to given capacity limits \citep{Borgwardt17}.


\textbf{Distance metrics.} 
Typically in clustering, a squared Euclidean distance metric is used and it corresponds to the the famous \textit{K-means clustering} \citep[see a recent review  by][]{Zhao18}. Although squared Euclidean has no physical interpretation and is not representative of travel, transportation or movement distance \citep{Murray98}, it can be utilized in some special occasions, for example the costs caused by fires can be expected to be quadratic with respect to the distance from the emergency center \citep{Zhou13}. However, when the aim is to directly minimize the physical distances between the demand points and the assigned facilities, the Euclidean distance metric is used. Furthermore,  in the discrete setting, the actual travel distances, or even the travel costs incurred, can be used in the objective function by pre-computing all the pairwise distances between the demand points and the facility candidates. 

==> text/OLD_choosing_k.tex <==
\subsection{Choosing the number of edge servers}

We first determine the optimal number of edge servers to be deployed. We apply the opening cost approach by selecting five different values for the $\lambda_k$ penalties, one of which is zero, and examine the value of the objective function with each possible value of $k$. We let $k$ range from 35 to 45 and with each $k$ we use 100 different initial values, chosen with k-means++. 

We assume the edge servers are identical and have an upper limit for the workload they can manage. Further, we set a lower limit for each server to balance the workload between the servers and to ensure no server capacity is wasted. We set the limits of one server to $[349, 648]$ which corresponds to a wide capacity range for the server. These limits correspond to $[\Bar{x} - 150, \Bar{x} + 150 ]$, with $\Bar{x} = 498.875$ the average workload for the servers in the $k = 40$ scenario. 

As the value of the opening cost penalty $\lambda_k$ is unknown in this experiment, we use five different values of $\lambda_k$ for each value of $k$. The resulting values of objective function allow us to evaluate the robustness of the deployment with respect to the penalty parameter and to decide accordingly which amount of servers is best suited for the data.

\begin{figure}
    \centering
    \includegraphics[width = 0.6\textwidth]{images/plot_shanghai_obj_lines.png}
    \caption{The value of the objective function with $k$ ranging from 35 to 45 and five different opening cost penalties: 0, 0.002, 0.004, 0.006 and 0.008. }
    \label{shanghai_obj_lines}
\end{figure}

The values of the objective function with the given variables, that is, the penalties and the number of centers, are listed in Fig. \ref{shanghai_obj_lines}. As expected, when no opening-cost is set, the value of the objective function decreases as $k$ increases. An exception, resulting from the lower capacity limit making it difficult to place servers optimally, can be seen at $k = 45$, with the objective function value increasing in all five penalty cases. An "elbow shape" can be seen at $k = 38$ with all penalty values, which indicates that number of servers provides a robust clustering. Another possible clustering choice is at $k = 44$, as it seems to have the lowest value of the objective function with small penalty values. 

% The most optimal placement of k = 35-45
%\begin{figure}
%    \centering
%    \includegraphics[width = %\textwidth]{images/plot_shanghai_k38.png}
%    \caption{The optimal placement of 38 edge servers in %the Shanghai region. The capacity limits for each %server is [349, 648].}
%    \label{fig:my_label}
%\end{figure}

==> text/Review.tex <==
\section{Extensions}

In the following subsections, we consider certain extensions common to location-allocation and partitional clustering and highlight their connections to model-based clustering. Such extensions include constraints on the locations of the centers, different distance metrics, weighted data points, capacity constraints on the clusters, different membership types, outliers, and selection of the number of centers.


\subsection{Constraints on the possible locations of the centers}
\label{centers}
So far, we have assumed that the centers can be located anywhere in the region of interest.  In location-allocation, problems where the facilities can be placed anywhere in the area are referred to as \textit{continuous location-allocation problems} or \textit{site generating problems} \citep{Brimberg08}. In clustering, algorithms with unrestricted placement of centers are referred to as \textit{virtual point prototype algorithms} \citep{Xiao12}. 

However, in both location-allocation and clustering, there are applications where the centers can be placed only on a predetermined set of points $\{p_1, p_2,... ,p_m\}$.  This can be achieved by including a constraint  
\[
\label{site}
c_j \in \{p_1, p_2,... ,p_m\} \quad \forall j
\]
to the optimization problem (\ref{loss}).

% https://doc.arcgis.com/en/arcgis-online/analyze/choose-best-facilities.htm

In location-allocation, this is a common constraint and the modified problem is referred to as the \textit{discrete location-allocation problem} or the \textit{site selection problem}. In clustering, there is less often a need to constrain the locations of the cluster centers, but if such a constraint is applied, the cluster centers are typically constrained to belong to the data points.  Thus, the constrained algorithms are referred to as \textit{actual point-prototype-based clustering algorithms} \citep{Xiao12}. %and one reason for their use is that they produce clusterings that are more robust for outliers (see Section~\ref{outliers} for further information) than the virtual point prototype algorithms.

In the following sections we will refer to the setup with constrained locations of centers as the discrete setting, and unconstrained locations as the continuous setting.

A third option for the cluster centers is that the locations of some centers may be fixed. In location-allocation, this is a typical setting, with new facilities being added to an existing network \citep[see e.g.][]{Rahman00}.  For clustering, such a variant may correspond e.g. to a setting where, based on prior information, it is known that there are clusters with centers in specific locations.% Such a setting  has been considered in model-based framework by \citep{Ganesalingam89}.



\subsection{Distance metrics}
\label{Distances}

Section~\ref{frameworks_intersection} described the connection between model-based clustering and the optimization problem (\ref{loss}) while applying the squared Euclidean, Manhattan and Euclidean distance metrics. However, the obtained methods are referred to differently depending on the framework and whether the continuous or discrete setting is applied. Here, we summarize the distance metrics along with the names of the algorithms in both settings and with different frameworks. We also consider other typical distance metrics considered in the frameworks. The metrics, along with the names of the methods, are listed in Table~\ref{table_distances}.

%In both clustering and location allocation, several different distance metrics can be used. To distances  that are applied both in location-allocation and in clustering frameworks with both continuous and discrete settings include $L_1$ norm (referred to as Manhattan distance, taxicab distance or rectilinear distance), $L_2$ norm i.e. Euclidean distance and the $L_2^2$ norm, i.e. the squared Euclidean distance. However, the algorithms utilizing these distances are referred to with different names depending on the framework, thus we  detail the distances along with the names of corresponding approaches in the different frameworks in Table~\ref{table_distances}. 

\textbf{Squared Euclidean distance.} As demonstrated in Section~\ref{classification_section}, minimizing the loss function  (\ref{loss}) in the continuous setting with the squared Euclidean distance metric corresponds to maximizing the classification maximum likelihood with an isotropic Gaussian distributions with equal variance and equal proportions. 

For the continuous setting in partitional clustering , the squared Euclidean distance metric corresponds to the famous \textit{K-means clustering} \citep[see a recent review  by][]{Zhao18}, whereas in the discrete setting, the metric corresponds to the \textit{K-medoid clustering} \citep{Kaufmann87}.

The squared Euclidean distance metric has no physical interpretation and is not representative of travel, transportation or movement distance \citep{Murray98}. It is thus less popular in location-allocation. However, in some special occasions, travel costs increase quadratically with the Euclidean distance. As an example, \citet{Zhou13} studied placing emergency service facilities, where the costs caused by fires can be expected to be quadratic with respect to the distance from the emergency center. Further, in the continuous setting, squared Euclidean distances may be used as approximations to Euclidean distances, as faster algorithms can be applied \citep{farahani2009}. %The goodness of the approximation depends on the distribution of the weights of the points, the more uneven weights the worse the approximation, and also on the symmetry of the groupings of the points, the more asymmetry in the groupings, the worse the approximation \citep{Watson72}. % oliko tähän joku viite?

\textbf{Euclidean distance.} Minimizing Euclidean distances in (\ref{loss}), on the other hand, corresponds to maximizing the classification maximum likelihood, assuming that the points have emerged from an isotropic Laplace distribution (\ref{classification_section}).  In partitional clustering, the Euclidean distance metric is more rarely used, and the approaches are referred to as \textit{Euclidean K-median} \citep[see e.g.][]{Kolliopoulos99} or simply \textit{K-median} \citep[see e.g.][]{Sariel04}. In the discrete setting, this approach, too, is referred to as \textit{K-medoid clustering} \citep{Kaufmann87}. 

In location-allocation, the Euclidean distance metric is often used, as the aim is to directly minimize the physical distances between the demand points and the assigned facilities. The discrete setting is referred to as the \textit{p-median method}  \citep[see reviews by][]{Mladenovic07, Daskin15} and the continuous setting as the \textit{multifacility Weber problem} \citep[see the review by][]{Brimberg08}. % Alternatively, \citet{Ahmadian19} merges clustering and location-allocation approaches and refers to the p-median problem as \textit{Euclidean K-median}.  

\textbf{Manhattan distance.} In model-based clustering, the Manhattan distance metric corresponds to assuming that the coordinates of each data point are generated from a univariate Laplace distribution \citep[see also][]{Cord06}. With the Manhattan distance metric, the method is referred to as \textit{K-median clustering} in the continuous setting and, in the discrete setting, again as K-medoid. In location-allocation this distance, also known as the city-block distance, may be used as a predictor of physical distance for example in an urban environment \citep{Brimberg08}.

%In the clustering framework,  the use of squared Euclidean distances in continuous setting corresponds to the famous K-means clustering  (see a recent review  by \cite{Zhao18}). If Manhattan  distances are utilized, the obtained method  is referred to as K-median clustering.  The Euclidean distances are more rarely used and the approaches are referred to as Euclidean K-median \citep[see e.g.][]{Kolliopoulos99}  or simply K-median \citep[see e.g.][]{}.
%In the discrete setting, the approaches obtained with all the three distances are referred to as  K-medoid clustering \citep{Kaufmann87}.

%On the other hand,  in location-allocation, typically the aim is to directly minimize the distances between the demand points and the assigned facilities and thus the Euclidean distances are most often used. The discrete setting is referred to as the p-median method  \citep[see reviews][]{Mladenovic07, Daskin15} and the continuous case as the multifacility Weber problem \citep[see review][]{Brimberg08}. However, there are articles merging clustering and location-allocation frameworks where a problem identical to the p-median problem is referred to as Euclidean K-median \cite{Ahmadian19}. The squared Euclidean distances  have no physical interpretation and is not representative of travel, transportation or movement distance \citep{Murray98} and are thus less often used. However, as in the continuous case, due to computational speed they may be used as an approximation to the Euclidean distances \citep{farahani2009}. The goodness of the approximation depends on the distribution of the weights of the points, the more uneven weights the worse the approximation, and also on the symmetry of the groupings of the points, the more asymmetry in the groupings, the worse the approximation.
%In some special occasions, however, the travel  costs increase quadratically with the Euclidean distance. As an example, \citet{Zhou13} locate emergency service facilities where the costs from fires can be expected to be quadratic with respect to the distance from the emergency center. 
%\citep[but see e.g.][]{Drezner99, Tafazzoli09}.

%In the model-based clustering, the use of Manhattan distances (i.e. K-median) corresponds to assuming that the $x$- and $y$-coordinates of each data point are generated from an univariate Laplace distribution \citep{Cord06} and Euclidean distances (i.e. the Weber problem) corresponds to assuming that the data is generated from isotropic multivariate Laplace distribution \footnote{There are several definitions for multivariate Laplace distribution, but here we refer to the one obtained as a special case of the multivariate exponential power distribution \citep{Naik06,Arslan10}}. The squared Euclidean distance, on the other hand,  corresponds to assuming that the data is generated from  a mixture of isotropic Gaussian distributions \citep{Raykov16, Bishop06}. 

\textbf{Mahalanobis distance.} The squared Euclidean distance metric implies an underlying assumption that the clusters are spherical, with similar shapes and sizes. With Euclidean or Manhattan distance metrics, remoteness from centers is not penalized as strongly. Still, if the aim is to detect the natural groupings in the data, both distances may produce sub-optimal clustering if the natural cluster sizes in the data are heterogeneous with, for example, elongated shapes.
A generalization that alleviates this problem is to apply the squared Mahalanobis distance metric, which allows elongated shapes and different spatial sizes for each cluster \citep{Cerioli05,Sung98}. This approach corresponds to assuming that the data of each cluster has emerged from an anisotropic multivariate Gaussian distribution. \citet{Sung98} referred to the approach as \textit{Elliptical K-means}. 

The challenge with the Mahalanobis distance metric is the difficulty in the initial estimation of the related covariance matrices. Several approaches have been proposed \citep{Xiang08, Melnykov14,Chokniwal16}. %For example \citep{Chokniwal16} utilized the K-means++ algorithm. 
Further, \citet{Lapidot18} recently highlighted convergence problems with K-means algorithms based on the Mahalanobis distance metric, and included regularization parameters for each cluster to achieve convergence.  The first proposed regularization penalizes large eigenvalues in the covariance matrices and the second one constrains the volumes of each cluster as constant. The Mahalanobis distance metric has also been combined with the K-median method by \citet{Ackermann10}, who specify a generalized K-median problem in the discrete setting, where an arbitrary dissimilarity measure is minimized and the Mahalanobis distance metric is used as an example.

\textbf{Threshold distance.} In location-allocation, typically Mahalanobis distance type generalization is not needed, as the aim is to minimize the travel distances regardless of the underlying structure of the data. However, different distance metrics have been proposed also in the location-allocation context. A loss function based on the Euclidean distance metric can be considered to minimize the average travel distance from the centers to the demand points. However, sometimes the aim may, instead, be to offer a facility within a given distance to as many demand points as possible. This corresponds to minimizing the percentage of demand  where the distance to the nearest facility exceeds a given threshold. In location-allocation literature this is referred to as the \textit{maximal coverage location problem} (MCLP) \citep{Church76,Church1986}. \citet{Church1986} have shown that the MCLP can be connected to the p-median problem by replacing the Euclidean distance metric with a thresholded distance metric where the distance is 0 if the Euclidean distance is under the given threshold and 1 if the threshold distance is exceeded.% MCLP can also be combined with a mandatory closeness requirement which states that for each point there must be a facility within distance $t$ while maximizing the percentage of demand within the $a$ threshold ($t>a$) \citep{Church74}. % ks. vielä mandatory etc, oli church et al...
% http://www.geog.ucsb.edu/~forest/G294download/MAX_COVER_RLC_CSR.pdf

\textbf{Distance matrix based distance.} Further, in location-allocation, Euclidean or Manhattan distance metrics are often only approximations of the actual travel distances or costs. In the discrete setting, the actual travel distances, or even the travel costs incurred, can be used in the objective function by pre-computing all the pairwise distances between the demand points and the facility candidates. Such approaches using pre-computed distances are also referred to as p-median problems \citep{Mladenovic07}, as the term p-median is not tied to the Euclidean distance metric. % Hence, in addition to travel distance, or time,  any distance function can be used. % See examples in  \citet{Gokbayrak17,Drezner91}.   % katso vielä läpi nämä viitteet ovatko diskreettejä vai jatkuvia?

%\begin{landscape}
\begin{table}[h!]
\begin{center}
\footnotesize
\caption{The distance metrics and the corresponding distributions and the referred methods in location-allocation and clustering.}
% \caption{The methods corresponding to Euclidean and squared Euclidean distances under the three frameworks.}
    \label{table_distances}
    \begin{tabular}{l l l l l l l} 
    \toprule
      \textbf{Name} & \textbf{Norm} & $\mathbf{d_{ij}}$ & \textbf{Distribution}  & \textbf{Center}  & \textbf{Location-Allocation} & \textbf{Clustering} \\
\midrule                
Manhattan& $L_1$  & \multirow{2}{*}{\begin{tabular}[t]{@{}l@{}}$|x_{i1}-y_{j1}|$\\ $ +|x_{i2}-y_{j2}|$  \end{tabular} }  & Laplace & Cont  & - & K-median \\ \cline{5-7}
(Taxicab, rectilinear) &  &             &         & Discr    & - & K-medoid\\
\midrule      
Euclidean & $L_2 $  & \multirow{4}{*}{\begin{tabular}[t]{@{}l@{}} $||x_i-y_j||=$\\ $\left((x_{i1}-y_{j1})^2 \right.$ \\  $\phantom{a}+\left.(x_{i2}-y_{j2})^2 \right)^{1/2}$ \end{tabular} }    & Multivariate   & Cont & Weber problem & Euclidean K-median \\   \cline{5-7}
         &  & & isotropic Laplace & Discr & p-median & K-medoid \\ 
           & & & & & \\
             & & & & & \\
\midrule
Squared  & $L_2^2$ &  $||x_i-y_j||^2$ & \multirow{2}{*}{ \begin{tabular}[t]{@{}l@{}}isotropic  \\ Gaussian \end{tabular}} &   Cont & - & K-means\\ \cline{5-7}
    Euclidean  &            &                  &            &    Discr & -  & K-medoid \\
    \midrule
Squared Mahalanobis & - &  $(x_i-y_j)\Sigma_j^{-1}(x_i-y_j)$ & \multirow{2}{*}{ \begin{tabular}[t]{@{}l@{}}Multivariate  \\ Gaussian \end{tabular}}   & Cont & - & \multirow{2}{*}{ \begin{tabular}[t]{@{}l@{}}Elliptical K-means \end{tabular}} \\
 & & & & & \\
\midrule
Threshold &  - & 
\multirow{3}{*}{$\begin{cases}
1  &  \text{ if } d_{ij} < a  \\
0  & \text{ otherwise } \end{cases}$ }    &  -    & Discr   & MCLP   & -    \\ \cline{5-7}
     &         &                         &     & Cont    & Continuous MCLP & -  \\
    &  & & & & \\      
    \midrule
Distance matrix    &  - & $D[ij]$ &- & Discr & p-median & - \\      
\bottomrule
            
    \end{tabular}
\end{center}
%\end{sidewaystable}
\end{table}
%\end{landscape}

\subsection{Weights}
\label{weights}

For location-allocation, each point $i$ is typically assigned a weight $w_i$ that corresponds to the amount of demand at that point such as the number of people living in an area. Weighted data points are rarer in clustering, but may similarly correspond to, e.g., the duplication of data \citep{Borgwardt17}. For such weighted optimization problems, the objective function (\ref{loss}) is replaced with
\begin{equation}
\label{loss_w}
    \argmin_{c_j, y_{i j}} \sum_{i = 1}^{n} \sum_{j = 1}^{k} w_id(x_i, c_j) y_{i j}.% +\lambda  \sum_{i = 1}^{n}  y_{i, k+1}
\end{equation}
 
\citet{Ackerman12} analyze clustering methods with respect to how they respond to the weighted data points, and summarize that K-means, K-median and K-medoid are weight separable. In other words, by modifying the weights of points, these algorithms separate any points to different clusters. Indeed, the effect of the distortion of a point $i$ in the objective function (\ref{loss}) is proportional to the weight $w_i$. Thus, such weight-sensitive techniques have two potentially conflicting considerations: the weight of the points and the geometry of the data. The points with heavy weights tend to attract the center even if they appear to be isolated.

Due to the tendency of heavy points to attract cluster centers, the weight can be used also for indicating points that are more important when locating a center. \citet{Wheeler19}, for example, create optimal police patrol areas by considering the number of calls weighted by the priority or duration of the call. Similarly, in case of clustering, \citet{Tseng07} interpret weights as an importance measure or, more generally, a prior measure which preferred or prohibited patterns of cluster selections. 

Also in model-based clustering, weights can be interpreted as measures of importance. \citet{Gebru16}, for example, consider Gaussian mixture models with weighted data. They interpret the weight of a point $i$ as its relevance, that is, the higher the weight of $i$, the stronger its impact on the clustering. They conclude that  $w_i$ can be considered as point-wise precision. In more detail, given a cluster, the points with a heavy weight are assumed to be drawn from a distribution which has a smaller variance than points with a small weight and are thus presumably located closer to the cluster center.

Above, weight is considered as an attribute of a data point. In clustering,  weights can more generally be assigned to the variables, i.e. the dimensions of the data points \citep[see a recent survey by ][]{deAmorim16}. Thus, some variables are considered more important than others in clustering. Typically, such weights are estimated during the clustering process. As our focus is on spatial data, the weights are only assigned to the points.

 \subsection{Capacities of facilities and sizes of clusters}
 \label{Capacity}

Clustering is often used for dissecting data into separate groupings for further processing or analysis. Such cases often aim at balanced clustering, where each cluster has a similar number of data points in each cluster, and too large or too small clusters are undesirable. Such balance may be desirable even if the “natural” clusters in the data were imbalanced \citep{Banerjee06}.

%% tästä oli banerjee viitannut kerns (ei vaikuttanut hyvältä viitteeltä) 
% katso kuitenkin:  Imbalanced K-Means: An algorithm to cluster imbalanced-distributed data, joka viittaa:  K-Means Clustering Versus Validation Measures: A Data-Distribution Perspective

Section~\ref{classification_section} showed that the minimization of (\ref{loss}) with the Euclidean, squared Euclidean and Manhattan distance metrics implies an assumption that the true clusters have equal proportions. This assumption was demonstrated also by \citet{Xiong08} who formally illustrate that K-means tends to produce nearly equal-sized clusters 
%%of relatively uniform sizes, 
even if the data has varying "true" cluster sizes. K-means and K-medians thus have a built-in tendency to produce balanced cluster sizes. However, neither guarantees balanced cluster sizes if the true sizes vary severely. Clustering methods that specifically aim at balancing the partitions are thus needed.

Clustering methods that aim at balance can be partitioned into two groups, balance constrained and balance driven approaches \citep{Malinen14}. In balance constrained clustering, the cluster size balance must be met, and the minimization of distances is only a secondary criterion. Balance driven clustering, on the other hand, is a compromise between balance and distance.

Several approaches have been proposed for both approaches. Balance constrained include \citet{Banerjee06},  \citet{Malinen14} and \citet{Elliott11}. Other constrained approaches include \citet{Hu18}, \citet{Zhu10} and \citet{Ganganath14}, where \citet{Hu18} constrain the size of the clusters only from below, and \citet{Zhu10} and \citet{Ganganath14} allow predefined size constraints to vary between clusters. 
%Balance-constrained \cite{Banerjee06}(scalable solution?),  \cite{Malinen14}(equal), \cite{Zhu10}(general constraints (not interval)), \cite{Hu18}(below (optimizes also k), \cite{Elliott11} (approximately equal (heuristic approach may be suboptimal?)), \cite{Baranwal17} (fixed (more like location-allocation paper?). 
% size restriction may also be proposed as a soft constraint that penalizes from large deviations  \cite{Li18,Liu17}.  %malisen väitöskirja
\citet{LI18} and \citet{Liu17} studied balance-driven clustering with a soft constraint that penalizes large deviations in cluster sizes. See also a recent survey on balanced data clustering algorithms by \citet{Gupta17}.

In model-based clustering, the constraints in the cluster size can be set as prior distributions. \citet{Jitta18} proposed flexible priors where each possible cluster size can be assigned with a prior probability. On the other hand,  \citet{Levine12} used a Poisson distribution as a prior distribution for the number of points in a cluster.

In location-allocation, the facilities may have a restricted amount of supplies, or capacity, that can not be surpassed. Thus the facilities must be placed and the demand allocated such that these capacity limits are followed. Such placement problems are referred to as \textit{capacitated location-allocation problems} and they include a hard upper capacity constraint,
\begin{equation}
\label{capacity_const}
 \sum_{i = 1}^{n} a_i y_{i j} \leq U \quad \forall j,
 \end{equation}
in the optimization problem (\ref{loss_w}).

In his seminal work, \citet{Cooper72} applied capacity constraints in the continuous setting, focusing on the Euclidean distance metric. Later, capacity constraints have been used with various distances both in the discrete (e.g. capacitated p-median problem, CPMP) and the continuous setting (e.g. capacitated multifacility Weber problem, CMWP). 

Note that in (\ref{capacity_const}) the constants $a_i$ may not be equal to the weights $w_i$. For example, \citet{Negreiros06} assign no weights in the objective function but use the demand only in the constraint to satisfy the capacity constraints. Further, also heterogeneous capacity constraints have been considered, as some applications have facilities with varying capacities \citep{Baranwal17, Liao08}.

Hard capacity constraints have also been proposed in the clustering framework by \citet{Mulvey84}, who assumed that the weights $w_i=1$ and coefficients $a_i=1$ for all $i$ and referred to the problem as the \textit{capacitated clustering problem} (CCP). Later, \citet{Negreiros06} used squared Euclidean distances in a continuous setting and referred to the problem as \textit{capacitated centered clustering problem} (CCCP). 

Location-allocation may also  aim for balance, as facilities with underused capacity may be undesirable. For example, \citet{Negreiros06} combine the aims of obeying the capacity constraints and balancing the data by setting a constraint that controls the number of points in each cluster, while \citet{Aras07} assume that the sum of demand assigned to a facility must be equal to its capacity.

Another possibility for combining balance and capacity constraints is to apply both a lower and an upper limit for the used capacity \citep{Borgwardt17} by including a constraint 
\[
 L \leq \sum_{i = 1}^{n} a_i y_{i j} \leq U \quad \forall j.
\]
In model-based clustering, such a hard capacity interval can be interpreted as a uniform prior distribution for used capacity \citep{Klami16}.

\subsection{Membership}
\label{membership}

Four different membership types are considered in both location-allocation and partitional clustering, namely, hard, uncertain, overlapping and fractional. 

\textbf{Hard membership.} 
The objective function (\ref{loss}) forces each point to be assigned to exactly one cluster. In clustering, this is referred to as hard or crisp clustering, and the membership of a point $i$ to center $j$ as hard membership or hard assignment. In location-allocation literature, this corresponds to an underlying assumption that each demand point is served by exactly one facility and thus referred to as single-sourcing.  
 
 \textbf{Uncertain membership.}
Uncertain membership means that a point can belong to many clusters in some degree.  
In model-based clustering with the mixture model (\ref{mixture}), each point is assigned the probabilities of belonging to each cluster. Thus, the memberships are of an uncertain type \textit{per se}.
In partitional clustering and location-allocation, an uncertain membership typically corresponds to fuzzy logic \citep{Klawonn03,Canos01}, where each point is assigned to each cluster with a membership degree that varies between 0 and 1. 

A fuzzy clustering version of the K-means is referred to as fuzzy c-means (FCM) \citep{Dunn73,Bezdek81}. The objective function is
\[
    \sum_{i = 1}^n \sum_{j = 1}^k u_{ij}^m \| x_{i} - c_{j} \|^2,
\]
where
\[
    u_{ij} = \frac{1}{\sum_{l=1}^k \left( \frac{\| x_i - c_j \|}{\| x_i - c_l  \|} \right)^\frac{2}{m - 1}}.
\]
The parameter $1 \leq m <\infty$ determines the level of fuzziness in the clustering, the larger the $m$ the fuzzier the result.  While a typical choice is $m=2$, limit $m=1$ corresponds to hard clustering, and as $m\rightarrow \infty$, the points have equal memberships for all clusters and the cluster centers converge to the center of the data \citep{Klawonn03}.

%In clustering framework there are several other approaches for expressing uncertainty in the membership.
Both model-based and FCM \citep{Bezdek81} apply a constraint requiring the memberships of a point $i$ to sum up to 1. \citet{Krishnapuram93} omit this constraint, and the resulting membership values may be interpreted as degrees of possibility of the points belonging to the clusters, i.e., the compatibilities of the points with the prototypes. \citet{Ben08} propose yet another alternative, referred to as \textit{probabilistic d-clustering}, that is based on an assumption that the probability of a point belonging to a cluster is inversely proportional to its distance from the cluster center. D-clustering was subsequently extended for unequal cluster sizes using the Mahalanobis distance metric \citep{Iyigun08}.
% PROBABILISTIC DISTANCE CLUSTERING ADJUSTED FOR CLUSTER SIZE (Mahalanobis)
 

\textbf{Overlapping membership.}
Overlapping membership means a point can be assigned to several centers.
In their review article, \citet{Cir15} divide partitional clustering approaches with overlapping membership into two groups: those with uncertain overlapping memberships, and those with hard overlapping memberships.
 
Fuzzy c-means can be extended to overlapping clustering by fixing a threshold such that all observations whose degrees of memberships exceed the threshold are assigned to the respective clusters. Similarly, in model-based clustering, overlapping membership could be implemented by assigning a threshold for the membership probability. However, there is a fundamental problem with such  straightforward modifications. Since both algorithms work in two phases, they initially  aim at optimizing an objective function under constraints that do not match with the expected overlapping structure of the clustering. Further,  there is a problem of choosing the suitable threshold \citep{Cleuziou08, Banerjee05}. 
 
There are  approaches that specifically combine uncertain membership clustering with the intuition of having overlapping clusters  \citep[see a review of][]{Cir15}. As an example, in Evidential c-means \citep{Masson08} all the possible combinations of clusters are evaluated and a mass of belief is allocated within each possible combination. In the model-based framework, \citet{Banerjee05} combine overlapping and uncertain memberships using a data generating function that omits the multinomial constraint. %that assumes that a point is generated from only one mixture component.  
 % Cleuziou yhteydessä banerjeen kanssa
 
 There are several approaches for hard overlapping membership. For instance, \citet{Cleuziou08} propose an overlapping K-means algorithm where each point is assigned to at least one cluster, and the aim is to minimize the squared distances between the points and the averages of the centers they are assigned to. Other partitional clustering approaches with overlapping membership are reviewed by \citet{Baadel16} and \citet{Cir15}. 
 
 In the location-allocation context, the view point for overlapping membership is different. Instead of identifying the points that should be assigned to several centers, either all or a predetermined subset of the points are assigned to several facilities, one of which is considered as a primary facility and the others as back-up facilities. This results, for example, in a more reliable system, where the assigned back-up facilities can be utilized in case the primary facility is not in use or is engaged with other demands. If back-up facilities are assigned for all points, such models are referred to as \textit{Q-coverage} (or \textit{K-coverage}) location models, and the constraint (\ref{const3}) is replaced with
 \[
 %\label{qcoverage}
 \sum_{j = 1}^{k} y_{i j} = Q \quad \forall i,
 \]
 where $Q$ is the number of assigned facilities \citep{Karatas16,Karatas17}. %Thus the membership of a point $i$ is 1 for $Q$ centers and 0 for others. 
% \citet{Karatas16} apply the Q-coverage requirement with the p-median and the maximal coverage location problems. %They compare the performance of the models with several different criteria including the mean distance to primary and back-up facilities.  In their experiments p-median outperforms  MCLP  in  four  criteria  out  of  five. Similar result were found by \citet{Winarso19} who compare p-median and MCLP in case of tobacco plantation production in Madura Island.
 

%http://web.b.ebscohost.com/ehost/pdfviewer/pdfviewer?vid=0&sid=2edc6c6b-8cd6-41d7-a6bf-d99a24f5849f%40pdc-v-sessmgr05
% backop!!

\textbf{Fractional membership.}  
% Separation index and partial membership for clustering
In fractional (also known as partial) clustering, a point can be shared by several clusters \citep{Borgwardt17}. Thus, the membership of a point $i$ to cluster $j$ is given by replacing the constraint (\ref{const2}) with a constraint
\begin{equation}
\begin{split}
\label{fractional}
y_{i j} \in [0, 1] \quad \forall i,j. \\
\end{split}
\end{equation}
In location-allocation, fractional  membership is referred to as multi-sourcing, and interpreted such that the demand of a point can be catered by several facilities.

If no capacity constraints are applied, each point is assigned to its closest center and thus, like with fuzzy c-means with $m=1$, fractional membership corresponds to hard membership. However, if capacity limits are applied, fractional membership allows a more flexible allocation of points into centers than the capacitated hard membership. In the extreme case, with hard membership, it may even be that the data points can not be partitioned according to given capacity limits \citep{Borgwardt17}.

In model-based clustering, \citet{Heller08} utilize fractional membership in the Bayesian framework, assuming that the memberships of points follow a Dirichlet distribution instead of the multinomial distribution as in the mixture models.  

Thus, with both uncertain and fractional memberships, a point can belong to several clusters with different degrees, with the degrees summing up to one. Still, these membership types are  different on a  conceptual level. Indeed, uncertainty on which center a point is assigned to is different from the certainty of a point belonging partially to several clusters \citep{Heller08}.  

The conceptual difference between overlapping and fractional clustering becomes evident with capacity constraints. In fractional clustering, fractions of the weight of a point are assigned to clusters, whereas in overlapping clustering the whole weight would be assigned to several points, thus requiring more capacity in the system.

% vertailupapereita
%Data Clustering with Cluster Size Constraints Using a Modified K-Means Algorithm
%   -- GMM paras fuzzy huonoin
%
% Comparative Study of K-means, Gaussian Mixture Model, Fuzzy C-means algorithms for Brain Tumor Segmentation
% fuzzy paras...

\subsection{Outliers}
\label{outliers}

With the aforementioned  membership types, each point is assigned to a cluster, albeit the assignment may be uncertain, overlapping or fractional. However, if a point does not seem to belong to any cluster, a forced assignment may distort information and the interpretation of the cluster it is assigned to \citep{Tseng07}. Similarly, in location-allocation, it may be economically essential to be allowed to exclude remote locations from service \citep{Charikar01}. 
Thus, in addition to allowing a point to be a member of several centers, it may be necessary to allow a point not to be a member of any center.  In both location-allocation and partitional clustering, such points that are left unassigned are referred to as outliers. Further, in partitional clustering, a partition where every point is assigned is referred to as complete clustering, and a partition where some points may be left unassigned is referred to as partial clustering \citep{Steinbach19}. 

The sensitiveness of the partition to the outliers depends on the method applied. For example, point prototype based clustering methods, where cluster centers are restricted to the data points, are more robust to outliers than the virtual point prototype based algorithms where the centers can be located anywhere \citep{Xiao12}. Further, the K-median method is known to be less sensitive to outliers than the K-means method \citep{Garcia10}, and can thus be considered as a robust alternative to K-means \citep{Raykov16}.
% Similar observations has also been made in the case of spatial clustering \citep{Murray98}.
 % From Murray:
 %This was found to be the case across values of p using numerous spatial data sets. Thus, the use of the squared distance measure results in inferior solutions when the data has spatial attributes. This should not be too surprising given that d2ij has no physical interpretation and is not representative of travel, transportation or movement distance
 
 % This is due to the fact that median is a more robust statistics against outliers than the mean.   This can be also explained through the implicit distribution assumption made, i.e. Laplace with heavier tails for K-median and light tailed Gaussian for K-means.
 Unlike the squared Euclidean distance metric, an Euclidean distance metric may mitigate the effect of outliers. Still, if outlier points are sufficiently far away from cluster centers, the outliers do distort the result even with the Euclidean distance metric \citep[cf.][]{Garcia10}. Thus, an explicit treatment of outliers is needed.
 
 %https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8261125
% Olukanmin K-means sharp menetelmän sensitiivisyys analyysi.

% fuzzy and robust:  https://www.ijcai.org/Proceedings/16/Papers/317.pdf

Outliers could be removed prior to the clustering by using some outlier detection method. However, the clustering structure may be highly dependent on the outliers, and on the other hand, the determination of the outliers depends on the clustering structure. Identifying the outliers should thus not be a separate step, but a part of the clustering process \citep{Liu19b}.

Outliers can be identified by determining the number of outliers prior to analysis, and iteratively assigning the most remote points as outliers. Such an approach has been proposed both in location-allocation \citep{Charikar01} and clustering \citep{Chawla13}. \citet{Whang15} combine outlier analysis with overlapping clustering by proposing an overlapping K-means algorithm where a fixed number of points is assigned to at least one cluster and a fixed number is not assigned at all.
Alternatively, outliers can be identified by keeping track of the distances of points to their nearest center.  \citet{Olukanmi17} determine such threshold iteratively.


%Alternatively, outliers can be identified by keeping track of the distances of points to their nearest centers. \citet{Charikar01} use a predetermined distance threshold, while \citet{Olukanmi17} determine the threshold iteratively.

A third alternative is to formulate the problem as a bi-criteria optimization, where a fixed penalty  is paid \citep{Charikar01,Tseng07} for each outlier point. Thus, the outliers can be considered to be assigned to a $k+1$'th cluster, with a penalty added to the loss function  (\ref{loss}).
\citet{Tseng07} further give this bi-criterion approach a model-based interpretation, pointing out that the penalty term  corresponds to assuming that the noise points are uniformly distributed, i.e., that they emerge from a homogeneous Poisson process.

% is replaced with
% \begin{equation}
% \label{outlier_penalty}
%\sum\sum + \lambda \sum_{i = 1}^{n}  .
% \end{equation}
 % In \citet{Ott14} computational speedups has been proposed for FLO.
% In Witten et al. a more flexible penalty term (millä lailla more flexible) can be used and in %Ott et al. also the number of clusters is simultaneously determined. 

%The parameter $\lambda$ dictates how expensive it is to assign a point as outiel, hence its value must be selected carefully.
%In case of location-allocation, the value  may be selected simply as a distance threshold over which the demand points are denied service. However, in case of clustering, the value may be more difficult to select  and  \citet{Tseng07} proposed a scaling for making the selection of $\lambda$ invariant under data scaling and the number of clusters. The scaling they propose is $\lambda=\lambda_0 \eta^p$ where for spatial data $\eta=H /\sqrt(k)$  with $H$ is the average pairwise distance among data points. For the squared Euclidean distance $p=2$, and for Euclidean distance $p=1$.     
%\[inline]{Onko tämä huomioitu siinä tsengissä, että se painokin vaikuttaa tässä?}

%\todo{tämä pitä laittaa kuntoon}
%Classification maximum likelihood can be written as
%\[
%l = \prod \cdot \frac{1}{s}
%\]
%If it is further assumed that each cluster has isotropic Gaussian distribution %with the same, known variance, the log likelihood is
%\[
%\frac{RSS}{\sigma^2} + \lambda
%\]
%then $\lambda_0=\sigma^2 \cdot \log A$, where $A$ is the area of the region of interest. This may provide further information for selecting the $\lambda$ parameter. 

%In this approach, a constant penalty is set for the outlier points, but \cite{witten13} proposed an approach where the location of an outlier point is assumed to consist of its true location and a degrading error term and the amount of penalty depends on the amount of error in the outlier points. %Thus the larger the error, the larger is the penalty.



%https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=7498276
% tuottaako dirichlet malli outliereita?
% https://www.researchgate.net/publication/228444163_Bayesian_Outlier_Detection_with_Dirichlet_Process_Mixtures


\subsection{Selection of the  number of centers}
\label{selectk}
Selecting the number of clusters is a widely studied topic in partitional clustering, with numerous approaches having been proposed over the years. Further, a number of reviews have been written on the topic. The review by \citet{Xu16} focuses on clustering methods in general, while \citet{Pham05} and \citet{Yuan2019} focus on approaches to K-means. 
%There are several variants of K-means that simultaneously cluster the data and determine the number of clusters namely the G-means \citep{Hamerly04}, the X-means \citep{Pelleg00} and iK-means \citep{Chiang10,Mirkin16}.   
%http://www.dcs.bbk.ac.uk/~mirkin/papers/n.pdf

In location-allocation, there are three typical approaches to determining the number of facilities. The first approach, referred to as the \textit{set covering problem}, places a minimal number of facilities by guaranteeing each demand point a facility within a given distance threshold \citep{Toregas73}. 

In the following two subsections, we will connect the two other approaches, namely the cost-effectiveness curve and the new facility opening cost, to the approaches utilized in clustering. 
%In the second approach, a curve, referred to as a cost-effectiveness curve, is drawn where the number of facilities is on the horizontal axis and the number of demand points within the aforementioned threshold distance from a facility is in the vertical axis. In the third approach, referred to as facility location problem, a bi-criterion optimization is utilized where a price is paid for opening each facility.

%The cost-effectiveness curve and opening cost approaches have also interpretations in clustering frameworks. Thus in the following subsections we will look into these connections further.  

%In this article, we focus on the latter two approaches, as similar approaches has been proposed also in the clustering framework. %AIC can be seen as setting an opening cost for a new facility whereas elbow resembles the cost effectiveness curve used in location-allocation.

\subsubsection{Opening cost}
The number of facilities can be selected by adding a penalty to the objective function  (\ref{loss}), referred to as the facility cost, for opening a new facility. The sums of weighted distances are then referred to as the service cost \citep{Charikar01}. The obtained optimization problem can be referred to as a \textit{facility location problem} or \textit{plant location problem} \citep{Arabani12}. 
  % \citep[][as e.g. in]{Carlo17}.
The cost of opening a new facility can depend on its location \cite[see e.g.][]{Azarmand09}, but in many applications, it is independent of location, and a predetermined fixed price $\lambda_k$ is paid for each opened facility. Thus the opening cost penalty corresponds to adding a penalty term  $\lambda_k k$ to the objective function (\ref{loss}).

Such a penalty for new centers has been proposed also in the partitional clustering framework \citep{Manning08}, but the interpretation of the approach is different. The sum of distances (\ref{loss}) and the penalty term $\lambda_k k$ are then considered to correspond to distortion and model complexity, respectively. A large number of centers corresponds to a small distortion but high model complexity, and vice versa for a small number of centers. Thus, the optimization problem can be seen as scalarized bi-objective optimization, where the parameter $\lambda_k$ controls the trade-off between the two aims. A small $\lambda_k$ produces partitions with a large number of clusters, and a large $\lambda_k$ produces partitions with a small number of clusters. The problem is thus converted to choosing the value of $\lambda_k$. 

% AIC as penalized likelihood..
One possible approach is to utilize information-theoretic measures that trade off distortion against model complexity. For example, Akaike's information criterion (AIC) and Bayesian information criterion (BIC) are defined as
\[
\text{AIC} = \argmin_{k} [-l+2q(k)], \quad  \quad  \text{BIC} = \argmin_{k} [-l+\log(n)q(k)], 
\]
where $l$ is the model maximum log-likelihood for $k$ clusters, and $q(k)$ is the number of parameters of a model with $k$ clusters \citep{Manning08}. 

For spatial K-means clustering with known variance this corresponds to
\[
  %  \label{AICBIC}
\text{AIC} =\argmin_{k} \left[\frac{\text{RSS}^*}{\sigma^2}+4k\right], \quad \quad \text{BIC} = \argmin_{k} \left[\frac{\text{RSS}^*}{\sigma^2}+2\log(n)k\right], 
\]
where $\text{RSS}^*$ is the minimized residual sum of squares with $k$ centers  (\ref{RSS2}).% \citep[cf.][]{Maindonald06}. % $\text{RSS}=\sum_{i = 1}^{n} \sum_{j = 1}^{k} w_i ||x_i -c^*_j||^2 y^*_{i j}$, where $c_j^*$ and $y_{ij}^*$ are the minimizers of (\ref{loss_w}) \citep[cf.][]{Maindonald06}.

%For K-means clustering this comes down to $K=2k$ in the case of spatial data.
%If the data emerge from isotropic Gaussian distributions with identical but unknown variances $\sigma^2$, AIC and BIC can be written as
%\[
%\text{AIC} = \log \text{RSS/n}+2K, \quad \quad  \text{BIC} %\log\text{RSS/n}+\log(n)K,
%\]
%where RSS is the minimized residual sum of squares (\ref{RSS2})   $\text{RSS}=\sum_{i = 1}^{n} \sum_{j = 1}^{k} w_i ||x_i -c^*_j||^2 y^*_{i j}$, where $c_j^*$ and $y_{ij}^*$ are the minimizers of (\ref{loss_w}) \citep{Maindonald06}. 

%However, if $\sigma^2$ is known, AIC \citep{Maindonald06} and BIC can be written as 
%\begin{equation}
%    \label{AICBIC}
%\text{AIC} = \frac{\text{RSS}}{\sigma^2}+2K, \quad \quad \text{BIC} = %\frac{\text{RSS}}{\sigma^2}+\log(n)K. 
%\end{equation}
% oliko maindonaldissa myös bic?

Thus, the opening cost approach with the squared Euclidean distance metric corresponds to clustering with AIC and BIC, assuming that the data points of each cluster follow a Gaussian distribution with known $\sigma^2$. The opening cost parameter for AIC is $\lambda_k=4\sigma^2$ and for BIC  $\lambda_k=2\log(n)\sigma^2$. 

AIC implies a smaller penalty term than BIC. Correspondingly, AIC is known to favor more complex models than BIC, with a higher number of parameters \citep{Theodoridis08}, corresponding here to more clusters. On the other hand, BIC tends to favor models that are too simple \citep{Theodoridis08}, that is, have too few clusters.

In practice, a $\lambda_k$ based on neither AIC nor BIC can be blindly followed in the selection of $\lambda_k$, with the ultimate choice of $\lambda_k$ remaining the responsibility of the model builder \citep{Manning08}. Nevertheless, they can be used as rough guidelines for $\lambda_k$, with AIC pointing towards the higher end in the spectrum of feasible $\lambda_k$'s, and BIC towards the lower end.
%In many occasions it is thus better to work directly with the general penalty parameter $\lambda_k k$, with the caveat that one must choose the value for the penalty \citep{Manning08}.

Further, mixture model based clustering can be connected to the opening cost approach if the number of clusters is assumed to be a random parameter that follows the Dirichlet distribution, i.e., if a Dirichlet process mixture model is applied \citep{Kulis12,Raykov16}. Furthermore, \citet{Kulis12} show that if the data for each cluster is assumed to have emerged from isotropic Gaussian distributions with the same variance for each cluster, the small-variance asymptotic of a Gibbs sampler for Dirichlet process mixture model corresponds to the minimization of $\text{RSS}+\lambda_k k$. 

%In the model-based clustering framework, a penalty for new centers is closely connected to the Dirichlet process mixture models that are extensions to the Gaussian mixture models where  the number of centers is assumed to be a random parameter that follows Dirichlet distribution \citep{Kulis12,Raykov16}.  \citet{Kulis12} show that if the data from each cluster is assumed to have emerged from spherical Gaussian distribution with the same variance for each cluster, the asymptotic of a Gibbs sampler for Dirichlet process mixture model corresponds minimization of $\text{RSS}+\lambda_k k$.  % tässä pitää avata enemmän tuota asymptotiikkaa, eli sigma lähestyy




%They also propose a K-means type algorithm, where the algorithm starts from one cluster centered to the mass  center of the data and a new cluster is formed when  a point is farther than $\lambda_k$  from its nearest center.   Such an interpretation for $\lambda_k$ as a threshold distance from center may help to choose its value also in the contexts of partitional clustering and location-allocation.


%[inline]{Statistical Inference: An Integrated Bayesian/Likelihood Approach, congdon}
% https://stackoverflow.com/questions/49118807/is-the-akaike-information-criterion-aic-unit-dependent
% jos on logaritmi uniteilla ei ole väliä!! 
% https://web.stanford.edu/class/stats202/content/lec13-cond.pdf

%Thus $\lambda_k$ can be interpreted as a threshold of the improvement in the distances for forming a new cluster, helping to choose the parameter. \[inline]{Onko muualla tuotu tuota tulkintaa esille? ja mminkä suhteen asymptotic small variance?}

%However, the Dirichlet prior tends to produce a small number of large clusters and (and a large number of small clusters) due to the "rich-get-richer" effect and thus Wallach et al. \cite{Wallach10} propose another type of prior...  And \citet{Miller} has shown that Dirichlet process is inconsistent on the estimation of the number of clusters

\subsubsection{Cost-effectiveness curve}

The MCLP approach draws a curve, referred to as the \textit{cost-effectiveness curve}, where the horizontal axis represents the number of facilities and the vertical axis represents the percentage of population within a predefined covering area from a facility \citep{Church74}. The number of facilities can then be chosen such that there is a reasonable trade-off between the covering percentage and the number of facilities. 

This approach resembles the "elbow" approach, often used in the clustering literature \citep{Kodinariya13}. The elbow approach draws a curve with the number of clusters on the horizontal axis and the minimum of the objective function on the vertical axis. The optimal number of clusters is then selected visually as the "elbow" of the curve, where increasing the number of clusters does not appear to produce a considerable decrease in the value of the objective function.
 
% A Comparison of Information Criteria in Clustering Based on Mixture of Multivariate Normal Distributions
% Degrees of Freedom and Model Selection for K-means Clustering


